Convolutional Residual Memory Networks

Very deep convolutional neural networks (CNNs) yield state of the art results on a wide variety of visual recognition problems. A number of state of the the art methods for image recognition are based on networks with well over 100 layers and the performance vs. depth trend is moving towards networks in excess of 1000 layers. In such extremely deep architectures the vanishing or exploding gradient problem becomes a key issue. Recent evidence also indicates that convolutional networks could benefit from an interface to explicitly constructed memory mechanisms interacting with a CNN feature processing hierarchy. Correspondingly, we propose and evaluate a memory mechanism enhanced convolutional neural network architecture based on augmenting convolutional residual networks with a long short term memory mechanism. We refer to this as a convolutional residual memory network. To the best of our knowledge this approach can yield state of the art performance on the CIFAR-100 benchmark and compares well with other state of the art techniques on the CIFAR-10 and SVHN benchmarks. This is achieved using networks with more breadth, much less depth and much less overall computation relative to comparable deep ResNets without the memory mechanism. Our experiments and analysis explore the importance of the memory mechanism, network depth, breadth, and predictive performance.

==> cutstuff.tex <==
\begin{table}[h!]
\centering
    \begin{tabular}{| l | l | l | l | l |}
    \hline
    Acc. (\%) & Method \\ \hline
    90.62 & Maxout Network \cite{goodfellow2013maxout} \\ \hline
    92.4  & Highway Network \cite{srivastava2015training} \\ \hline
    93.45 & ELU Network \cite{clevert2015fast} (18 layers) \\ \hline
    93.03 & Residual Network (56 layers) \cite{he2015deep} \\ \hline
    93.57 & Residual Network (110 layers) \cite{he2015deep} \\ \hline
%96.53 & Fractional Max-pooling \cite{graham2014fractional}
94.16 & LSUV Initialization Method \cite{DBLP:journals/corr/MishkinM15} \\ \hline
\hline
     \textbf{94.6} & Our CRMN (56 layers)  \\ \hline
    \end{tabular}
\caption{List of accuracies of various classification methods on CIFAR-10}
\label{tab:cifar10}
\end{table}

\begin{table}[h!]
\centering
    \begin{tabular}{| l | l | l | l | l |}
    \hline
    Acc. (\%) & Method \\ \hline
     67.61 & Highway Network \cite{srivastava2015training} (100 layers) \\ \hline
     71.14 & Maxout Network \cite{goodfellow2013maxout}  \\ \hline
     72.34 & LSUV Initialization Method \cite{DBLP:journals/corr/MishkinM15} \\ \hline
%     72.60 & Bayesian Optimization \cite{snoek2015scalable}  \\ \hline
     74.84 & Residual Network \cite{he2015deep} (164 layers) \cite{he2016identity}    \\ \hline
     75.72 & ELU Network \cite{clevert2015fast} (18 layers)  \\ \hline
%   CRMN[ours] & 76.60 \\ \hline
% 74.84 25.16 164 layer - numbers are from newer ResNet paper
% 75.67 24.33 164 preactivation
%     77.29 & Pre-activation ResNet \cite{he2016identity} (1001 layers - \emph{arXiv result, not yet peer reviewed}) \\ \hline 
\hline
     \textbf{77.43} & Our CRMN (32 layers)  \\ \hline
    \end{tabular}
\caption{List of accuracies of various classification methods on CIFAR-100}
\label{comparison}
\end{table}


